A Revisit to the Decoder for Camouflaged Object Detection

Camouflaged object detection (COD) aims to generate a fine-grained segmentation map of camouflaged objects hidden in their background. Due to the hidden nature of camouflaged objects, it is essential for the decoder to be tailored to effectively extract proper features of camouflaged objects and extra-carefully generate their complex boundaries. In this paper, we propose a novel architecture that augments the prevalent decoding strategy in COD with Enrich Decoder and Retouch Decoder, which help to generate a fine-grained segmentation map. Specifically, the Enrich Decoder amplifies the channels of features that are important for COD using channel-wise attention. Retouch Decoder further refines the segmentation maps by spatially attending to important pixels, such as the boundary regions. With extensive experiments, we demonstrate that ENTO shows superior performance using various encoders, with the two novel components playing their unique roles that are mutually complementary.

==> tabs/table4.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{\textbf{Importance of high resolution input in COD.} Performances of MSRA-B and NC4K datasets based on different input resolutions are shown. The last column denotes the performance improvements in MSRA-B and NC4K, using higher resolution images as input.
%of $\mathcal{L}_\text{KD}$ and $\mathcal{L}_\text{CL}$ shows the best performance.
}
%\vspace{-3mm}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{c|cc|cc|cc}
    \toprule
    % $\mathcal{L}_{MSE}$ & $\mathcal{L}_{KD}$ & $\mathcal{L}_{CL}$  & mAP (\%)\\
     & \multicolumn{2}{c|}{$160\times160$}   &   \multicolumn{2}{c|}{$320\times320$} &  \multicolumn{2}{c}{\textbf{Improvements}} \\
    \midrule
    Metrics & MSRA & NC4K & MSRA & NC4K & MSRA & NC4K \\
    % Assist & Refine & Detail & ${S_\alpha}$ ↑ & ${F_\beta^w}$ ↑ & ${E_\phi}$ ↑ & ${M}$ ↓\\
    \midrule
    ${S_\alpha}$ ↑ &  0.902  & 0.838 & 0.915 & 0.888 & 0.013 & \textbf{0.050} \\
    ${F_\beta^w}$ ↑&  0.870  & 0.743 & 0.894 & 0.834 & 0.024 & \textbf{0.091} \\
    ${E_\phi}$ ↑   &  0.925  & 0.890 & 0.938 & 0.932 & 0.013 & \textbf{0.042} \\
    ${M}$ ↓        &  0.044  & 0.049 & 0.039 & 0.032 & 0.005 & \textbf{0.017} \\
    % \hline
    \bottomrule
\end{tabular}
% }
\vspace{-3ex}
\label{tab:multiscale_ablation}
\end{table}
